Alternating Direction Method of Multipliers for Decomposable Saddle-Point Problems

Saddle-point problems appear in various settings including machine learning, zero-sum stochastic games, and regression problems. We consider decomposable saddle-point problems and study an extension of the alternating direction method of multipliers to such saddle-point problems. Instead of solving the original saddle-point problem directly, this algorithm solves smaller saddle-point problems by exploiting the decomposable structure. We show the convergence of this algorithm for convex-concave saddle-point problems under a mild assumption. We also provide a sufficient condition for which the assumption holds. We demonstrate the convergence properties of the saddle-point alternating direction method of multipliers with numerical examples on a power allocation problem in communication channels and a network routing problem with adversarial costs.

==> backup.tex <==



%\begin{equation}
     \mathcal{L} (\varminimizeritr{*}, \varmaximizeritr{*}, \auxvarminimizeritr{*}, \auxvarmaximizeritr{*}, \dualvarminimizer, \dualvarmaximizer) \leq \bar{\mathcal{L}}(\varminimizeritr{*}, \varmaximizeritr{*}, \auxvarminimizeritr{*}, \auxvarmaximizeritr{*}, \dualvarminimizer, \dualvarmaximizer, \mu_{\minimizer}, 0, \mu_{\minimizer, 1}, \ldots, \mu_{\minimizer, N}, 0, \ldots, 0) 
\end{equation} since \(G_{\minimizer,i}\varminimizerblockitr{i}{*} + h_{\minimizer,i} \leq 0\), \(G_{\minimizer,i}\auxvarminimizeritr{*} + h_{\minimizer,i} \leq 0\), and \(\mu_{\minimizer}, \mu_{\minimizer, 1}, \ldots, \mu_{\minimizer, N} \geq 0\). Similarly,




This implies that strong duality holds for the Lagrangian, i.e., 
\begin{equation}
    \min_{\substack{\varminimizer \in \spaceminimizerblock{1} \times \ldots \times \spaceminimizerblock{N} \\ \auxvarminimizer \in \spaceminimizer \\ \dualvarmaximizer}} \ 
    \max_{\substack{\varmaximizer \in \spacemaximizerblock{1} \times \ldots \times \spacemaximizerblock{N} \\ \auxvarmaximizer \in \spacemaximizer \\ \dualvarminimizer}} \mathcal{L} (\varminimizer, \varmaximizer, \auxvarminimizer, \auxvarmaximizer, \dualvarminimizer, \dualvarmaximizer) =   
    \max_{\substack{\varmaximizer \in \spacemaximizerblock{1} \times \ldots \times \spacemaximizerblock{N} \\ \auxvarmaximizer \in \spacemaximizer \\ \dualvarminimizer}} \ \min_{\substack{\varminimizer \in \spaceminimizerblock{1} \times \ldots \times \spaceminimizerblock{N} \\ \auxvarminimizer \in \spaceminimizer \\ \dualvarmaximizer}} \mathcal{L} (\varminimizer, \varmaximizer, \auxvarminimizer, \auxvarmaximizer, \dualvarminimizer, \dualvarmaximizer) 
\end{equation}


    \\
     &= \dualvarmaximizeritr{k+1}
    \\
    &=\frac{\partial  (\dualvarmaximizeritr{k+1})^{\top}\auxvarmaximizer }{\partial \varmaximizer}\Biggr|_{\substack{\varmaximizer = \auxvarmaximizeritr{k+1}}}
    \\
    &
    
    
    
    Saddle-point ADMM works in the following way:
\begin{enumerate}
\item    Initialize \(\varminimizeritr{0}, \varmaximizeritr{0}, \auxvarminimizeritr{0}, \auxvarmaximizeritr{0}, \dualvarminimizeritr{0}, \dualvarmaximizeritr{0}\) such that \(\varminimizeritr{0} \in \spaceminimizerblock{1} \times \ldots \times \spaceminimizerblock{N}\), \(\varmaximizeritr{0} \in \spacemaximizerblock{1} \times \ldots \times \spacemaximizerblock{N}\), \(\auxvarminimizeritr{0} \in \spaceminimizer\), and \(\auxvarmaximizeritr{0} \in \spacemaximizer\).
\item For \(k = 1, 2, \ldots\) repeat
\begin{enumerate}
        \item  Set \(\varminimizeritr{k+1}, \varmaximizeritr{k+1} \) as \[ \arg \min_{\varminimizer } \ \max_{\varmaximizer } \ \hat{\mathcal{L}}(\varminimizer, \varmaximizer, \auxvarminimizeritr{k}, \auxvarmaximizeritr{k}, \dualvarminimizeritr{k}, \dualvarmaximizeritr{k}) \] \label{step:saddleADMMvarupdate}
        \item  \[\auxvarminimizeritr{k+1} = \arg \min_{\auxvarminimizer} \hat{\mathcal{L}}(\varminimizeritr{k+1}, \varmaximizeritr{k+1}, \auxvarminimizer, \auxvarmaximizeritr{k}, \dualvarminimizeritr{k}, \dualvarmaximizeritr{k})\]
         \[\auxvarmaximizeritr{k+1} = \arg \max_{\auxvarmaximizer} \hat{\mathcal{L}}(\varminimizeritr{k+1}, \varmaximizeritr{k+1}, \auxvarminimizeritr{k+1}, \auxvarmaximizer, \dualvarminimizeritr{k}, \dualvarmaximizeritr{k})\] \label{step:saddleADMMauxvarupdate}

        \item \[\dualvarminimizeritr{k+1} = \dualvarminimizeritr{k} + \dualstepsizeminimizer(\varminimizeritr{k+1} - \auxvarminimizeritr{k+1})\]
        \[\dualvarmaximizeritr{k+1} = \dualvarmaximizeritr{k} + \dualstepsizemaximizer(\varmaximizeritr{k+1} - \auxvarmaximizeritr{k+1})\] \label{step:saddleADMMdualupdate}

\end{enumerate}

\end{enumerate}



ADMM for \eqref{prob:onlyminwithaux} works in the following way:
\begin{enumerate}
    \item Initialize \(\varminimizeritr{0}, \auxvarminimizeritr{0}, \dualvarminimizeritr{0}\) such that \(\varminimizeritr{0} \in \spaceminimizerblock{1} \times \ldots \times \spaceminimizerblock{N}\), \(\auxvarminimizeritr{0} \in \spaceminimizer\).
    \item For \(k = 1, 2, \ldots\) repeat
    \begin{enumerate}
        \item  \(\varminimizeritr{k+1} = \arg \min_{\varminimizer }  \ \hat{\mathcal{K}}(\varminimizer, \auxvarminimizeritr{k},  \dualvarminimizeritr{k}) .\)  \label{step:minADMMvarupdate}
    
    \item \(\auxvarminimizeritr{k+1} = \arg \min_{\auxvarminimizer} \ \hat{\mathcal{K}}(\varminimizeritr{k+1},  \auxvarminimizer, \dualvarminimizeritr{k}).\) \label{step:minADMMauxvarupdate} 
    
    \item \(\dualvarminimizeritr{k+1} = \dualvarminimizeritr{k} + \dualstepsizeminimizer(\varminimizeritr{k+1} - \auxvarminimizeritr{k+1})\) \label{step:minADMMdualvarupdate}
    \end{enumerate}
\end{enumerate} 



    \\
    &= \frac{\partial  \sum_{i=1}^{N} \funcblock{i}(\varminimizerblock{i}, \varmaximizerblock{i}) }{\partial \varminimizer}\Biggr|_{\substack{\varminimizer = \varminimizeritr{k+1}}} + \dualvarminimizeritr{k} + \dualstepsizeminimizer (\varminimizeritr{k+1} - \auxvarminimizeritr{k})
    \\
    &=\frac{\partial  \sum_{i=1}^{N} \funcblock{i}(\varminimizerblock{i}, \varmaximizerblock{i}) }{\partial \varminimizer}\Biggr|_{\substack{\varminimizer = \varminimizeritr{k+1}}} + \dualvarminimizeritr{k+1} - \dualstepsizeminimizer (\auxvarminimizeritr{k+1} - \auxvarminimizeritr{k})
    \\
    &=\frac{\partial  \sum_{i=1}^{N} \funcblock{i}(\varminimizerblock{i}, \varmaximizerblock{i}) + (\dualvarminimizeritr{k} - \dualstepsizeminimizer (\auxvarminimizeritr{k+1} - \auxvarminimizeritr{k}))^{\top} \varminimizer }{\partial \varminimizer}\Biggr|_{\substack{\varminimizer = \varminimizeritr{k+1}}}
    \\
    &


 
    \\&= - \dualvarminimizeritr{k} - \dualstepsizeminimizer (\varminimizeritr{k+1} - \auxvarminimizeritr{k+1}) = - \dualvarminimizeritr{k+1}
    \\
    &
    
    =\frac{\partial  -(\dualvarminimizeritr{k+1})^{\top}\auxvarminimizer }{\partial \varminimizer}\Biggr|_{\substack{\varminimizer = \auxvarminimizeritr{k+1}}}
    
    
    
    Due to the saddle point assumption, we have \[\mathcal{L}(\varminimizeritr{*}, \varmaximizeritr{k+1}, \auxvarminimizeritr{*}, \auxvarmaximizeritr{k+1}, \dualvarminimizeritr{*}, \dualvarmaximizeritr{*}) \leq \mathcal{L}(\varminimizeritr{*}, \varmaximizeritr{*}, \auxvarminimizeritr{*}, \auxvarmaximizeritr{*}, \dualvarminimizeritr{*}, \dualvarmaximizeritr{*}).\] Since \(\optvalue = \mathcal{L} (\varminimizeritr{*}, \varmaximizeritr{*}, \auxvarminimizeritr{*}, \auxvarmaximizeritr{*}, \dualvarminimizeritr{*}, \dualvarmaximizeritr{*})\) and \(\varminimizeritr{*} = \auxvarminimizeritr{*}\), we have \[ \optvaluemaximizeritr{k+1} - (\dualvarmaximizeritr{*})^{\top} (\varmaximizeritr{k+1} - \auxvarmaximizeritr{k+1})\leq \optvalue.\] Using \(\primalresidualmaximizeritr{k+1} = \varmaximizeritr{k+1} - \auxvarmaximizeritr{k+1}\) and rearranging the terms, we get 
\begin{equation} \label{ineq:maximizerconvergesfrombottomproof}
    \optvaluemaximizeritr{k+1} - \optvalue  \leq (\dualvarmaximizeritr{*})^{\top} \primalresidualmaximizeritr{k+1}.
\end{equation}


\begin{align}
    &\mathcal{L} (\varminimizeritr{*}, \varmaximizer, \auxvarminimizeritr{*}, \auxvarmaximizer, \dualvarminimizeritr, \dualvarmaximizeritr{*}) \nonumber
    \\
    &\leq \mathcal{L} (\varminimizeritr{*}, \varmaximizeritr{*}, \auxvarminimizeritr{*}, \auxvarmaximizeritr{*}, \dualvarminimizeritr, \dualvarmaximizeritr{*})  \label{saddlebarlagrangianmaximizerfreeminimizer}
    \\
    &\leq     \mathcal{L} (\varminimizeritr{*}, \varmaximizeritr{*}, \auxvarminimizeritr{*}, \auxvarmaximizeritr{*}, \dualvarminimizeritr, \dualvarmaximizer) \nonumber
\end{align}

\begin{align}
    &\mathcal{L} (\varminimizeritr{*}, \varmaximizeritr{*}, \auxvarminimizeritr{*}, \auxvarmaximizeritr{*}, \dualvarminimizer, \dualvarmaximizer) \nonumber
    \\
    &\leq \mathcal{L} (\varminimizeritr{*}, \varmaximizeritr{*}, \auxvarminimizeritr{*}, \auxvarmaximizeritr{*}, \dualvarminimizeritr{*}, \dualvarmaximizer) \label{saddlebarlagrangianminimizerfreemaximizer}
    \\
    &\leq     \mathcal{L} (\varminimizer, \varmaximizeritr{*}, \auxvarminimizer, \auxvarmaximizeritr{*}, \dualvarminimizeritr{*}, \dualvarmaximizer) \nonumber
\end{align}

\begin{align*}
    \hat{\mathcal{L}}&(\varminimizer, \varmaximizer, \auxvarminimizer, \auxvarmaximizer, \dualvarminimizer, \dualvarmaximizer) =
    \\
    &  \sum_{i=1}^{N} \left(\funcblock{i}(\varminimizerblock{i}, \varmaximizerblock{i}) + \indicatorfunc{\spaceminimizerblock{i}}  (\varminimizerblock{i}) - \indicatorfunc{\spacemaximizerblock{i} }(\varmaximizerblock{i}) \right)
    \\
    &+ \dualvarminimizer^{\top}(\varminimizer - \auxvarminimizer) + \frac{\dualstepsizeminimizer}{2} \ltwonorm{\varminimizer - \auxvarminimizer} + \indicatorfunc{\spaceminimizer}(\auxvarminimizer) 
    \\
    &- \dualvarmaximizer^{\top}(\varmaximizer - \auxvarmaximizer) - \frac{\dualstepsizemaximizer}{2} \ltwonorm{\varmaximizer - \auxvarmaximizer}  - \indicatorfunc{\spacemaximizer}(\auxvarmaximizer).
\end{align*}

\begin{align*}
&  \sum_{i=1}^{N} \left(\funcaltblock{i}(\varminimizerblock{i}) + \indicatorfunc{\spaceminimizerblock{i}}  (\varminimizerblock{i}) \right)
    \\
    &+ \dualvarminimizer^{\top}(\varminimizer - \auxvarminimizer) + \frac{\dualstepsizeminimizer}{2} \ltwonorm{\varminimizer - \auxvarminimizer} + \indicatorfunc{\spaceminimizer}(\auxvarminimizer)
\end{align*}

==> backupcommands.tex <==



\newcommand{\varminimizeritr}[1]{\textcolor{blue}{\ensuremath{x_{\minimizer}^{#1}}}}
\newcommand{\varmaximizeritr}[1]{\textcolor{red}{\ensuremath{x_{\maximizer}^{#1}}}}
\newcommand{\auxvarminimizeritr}[1]{\textcolor{blue}{\ensuremath{z_{\minimizer}^{#1}}}}
\newcommand{\auxvarmaximizeritr}[1]{\textcolor{red}{\ensuremath{z_{\maximizer}^{#1}}}}
\newcommand{\dualvarminimizeritr}[1]{\textcolor{blue}{\ensuremath{\dualvar_{\minimizer}^{#1}}}}
\newcommand{\dualvarmaximizeritr}[1]{\textcolor{red}{\ensuremath{\dualvar_{\maximizer}^{#1}}}}
\newcommand{\primalresidualminimizeritr}[1]{\textcolor{blue}{\ensuremath{r_{\minimizer}^{#1}}}}
\newcommand{\primalresidualmaximizeritr}[1]{\textcolor{red}{\ensuremath{r_{\maximizer}^{#1}}}}
\newcommand{\dualresidualminimizeritr}[1]{\textcolor{blue}{\ensuremath{s_{\minimizer}^{#1}}}}
\newcommand{\dualresidualmaximizeritr}[1]{\ensuremath{s_{\maximizer}^{#1}}}
\newcommand{\varminimizerblockitr}[2]{\textcolor{blue}{\ensuremath{x_{\minimizer, #1}^{#2}}}}
\newcommand{\varmaximizerblockitr}[2]{\textcolor{red}{\ensuremath{x_{\maximizer, #1}^{#2}}}}
\newcommand{\auxvarminimizerblockitr}[2]{\textcolor{blue}{\ensuremath{z_{\minimizer, #1}^{#2}}}}
\newcommand{\auxvarmaximizerblockitr}[2]{\textcolor{red}{\ensuremath{z_{\maximizer, #1}^{#2}}}}
\newcommand{\dualvarminimizerblockitr}[2]{\textcolor{blue}{\ensuremath{\dualvar_{\minimizer, #1}^{#2}}}}
\newcommand{\dualvarmaximizerblockitr}[2]{\textcolor{red}{\ensuremath{\dualvar_{\maximizer, #1}^{#2}}}}
\newcommand{\primalresidualminimizerblockitr}[2]{\textcolor{blue}{\ensuremath{r_{\minimizer, #1}^{#2}}}}
\newcommand{\primalresidualmaximizerblockitr}[2]{\textcolor{red}{\ensuremath{r_{\maximizer, #1}^{#2}}}}
\newcommand{\dualresidualminimizerblockitr}[2]{\textcolor{blue}{\ensuremath{s_{\minimizer, #1}^{#2}}}}
\newcommand{\dualresidualmaximizerblockitr}[2]{\textcolor{red}{\ensuremath{s_{\maximizer, #1}^{#2}}}}
\newcommand{\optvalueminimizeritr}[#1]{\textcolor{blue}{(p^{*}_{\minimizer})^{#1}}}
\newcommand{\optvaluemaximizeritr}[#1]{\textcolor{red}{(p^{*}_{\maximizer})^{#1}}}


==> power_allocation_residuals.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}[scale=0.75]

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
width=4.164in,
height=1.45in,
tick align=outside,
tick pos=left,
legend cell align={left},
legend columns=2, 
legend style={fill opacity=1, draw opacity=1, text opacity=1},
		xmajorgrids,
		ymajorgrids,
		yminorgrids,
x grid style={darkgray176},
xlabel={\(k\) (Iteration)},
log basis y={10},
xmin=0, xmax=100,
xtick style={color=black},
ymode=log,
y grid style={darkgray176},
ylabel={Total Residual Norm},
ymin=0.001, ymax=100,
ytick style={color=black}
]
\addplot [line width=2pt, black]
table {%
0 2000009.48683298
1 85.3814968245463
2 72.5092073120207
3 51.9369380391709
4 40.9860629520718
5 33.5850627972242
6 28.3115345575348
7 24.3534675466291
8 21.2772723397209
9 18.7840765084751
10 16.7346730356417
11 15.0207706704766
12 13.5137012433998
13 12.2233117893713
14 11.0652953729162
15 10.0782783500135
16 9.21157657136196
17 8.3972782509855
18 7.67959938406554
19 7.02271678069814
20 6.45174806684295
21 5.92996509659491
22 5.44071118013577
23 4.99914184637625
24 4.63519500950485
25 4.25198898601991
26 3.9496340074247
27 3.60130944653386
28 3.34872948538242
29 3.05354619827157
30 2.84940227945513
31 2.61503495061441
32 2.38199112755902
33 2.19292044800276
34 2.12577549087997
35 1.98305911149269
36 1.92948380118863
37 1.84672041597668
38 1.79774760686401
39 1.73728847004209
40 1.63293164573046
41 1.56762383459822
42 1.53257394172651
43 1.43746925112047
44 1.39585398885833
45 1.36851506941782
46 1.2934526196435
47 1.25546332100704
48 1.20275952075617
49 1.17208724750868
50 1.13789858343653
51 1.07386159371735
52 1.02372074414012
53 0.950560150680429
54 0.966412282218941
55 0.908307034404181
56 0.857887354204559
57 0.850994372202121
58 0.781921118737845
59 0.79274596148704
60 0.77355665957145
61 0.714280549861423
62 0.711746810186818
63 0.627176226400883
64 0.621686906660636
65 0.610503541323431
66 0.576887669691123
67 0.551207193912849
68 0.537037319448759
69 0.543296226332239
70 0.508180250689071
71 0.488029113326615
72 0.424072059856524
73 0.41700410034621
74 0.432809823412431
75 0.399218433939671
76 0.38407019940592
77 0.376128574309897
78 0.340624839253608
79 0.341104430110216
80 0.301765968321025
81 0.250744381845707
82 0.236793324509073
83 0.247102279403718
84 0.217572825530995
85 0.199962208826335
86 0.208296399375141
87 0.216787345209985
88 0.21155787144965
89 0.199533703769181
90 0.176810049795061
91 0.178688029992207
92 0.180502445368096
93 0.14542189570802
94 0.149666909076814
95 0.171353609037068
96 0.172956407083849
97 0.161252866724608
98 0.163071236714125
99 0.165260912789434
};
\addlegendentry{\(\dualstepsizeminimizer=\dualstepsizemaximizer=0.001\)}
\addplot [line width=2pt, purple]
table {%
0 2000009.48683298
1 30.5903893611778
2 12.4253524174212
3 6.2966495709485
4 3.40065426152502
5 1.81125470184572
6 1.18364943870229
7 0.859952469173617
8 0.568824468636748
9 0.381749461844574
10 0.311897965688101
11 0.204132252374323
12 0.11895870863723
13 0.0841909075656914
14 0.049540847562378
15 0.0644053795145617
16 0.0439449565018557
17 0.0551684215965055
18 0.0735012022735367
19 0.0139742912601109
20 0.0156259234188147
21 0.021739656778275
22 0.0287636783751422
23 0.0247700138016415
24 0.0165931995884292
25 0.0385435714701772
26 0.0479747781594825
27 0.0338113208474037
28 0.020428428420461
29 0.00416479424741912
30 0.00629500567996647
31 0.00743796986935059
32 0.0104371256661254
33 0.0130015297790414
34 0.0171758932626139
35 0.0237202961552932
36 0.0307497225496119
37 0.0426605219587394
38 0.0818417594520721
39 0.0115339046638214
40 0.0119740612359213
41 0.0162341398376056
42 0.0219194662906879
43 0.0188493305115826
44 0.0248327401247851
45 0.00306909887314698
46 0.020128015597854
47 0.0125145882461714
48 0.0216613372334859
49 0.0314707465961653
50 0.0408428851168025
51 0.0272063363139913
52 0.0142779355274322
53 0.0205655302008577
54 0.0243990670848017
55 0.0182132190699184
56 0.0212295714477917
57 0.0240553543331677
58 0.0275896149306313
59 0.0222260383482968
60 0.0280086680678243
61 0.0393524310070066
62 0.0414515473157198
63 0.0175239793979335
64 0.0104909239586306
65 0.0177592127970107
66 0.0224166664839336
67 0.0293866372063376
68 0.0272817402173044
69 0.0300109837556609
70 0.0102304719776994
71 0.0275831753750359
72 0.0125305113805498
73 0.0375289785646042
74 0.0617600535537307
75 0.033114383102992
76 0.0138692236389058
77 0.018538890804948
78 0.0241677526619657
79 0.0224439059480176
80 0.0304405845796772
81 0.0352147941673664
82 0.054550490270922
83 0.0262441358809114
84 0.021832865019444
85 0.0300250038984532
86 0.0374708416021886
87 0.0730649339018044
88 0.0181838740062775
89 0.0193480742365966
90 0.0171515078699611
91 0.0176501791128943
92 0.0271873947059498
93 0.0340569425648995
94 0.0502420451707856
95 0.0873063667491427
96 0.0457408037223843
97 0.0536923893226155
98 0.0535403304763296
99 0.0289674411038986
};
\addlegendentry{\(\dualstepsizeminimizer=\dualstepsizemaximizer=0.01\)}
\addplot [line width=2pt, green!50!black]
table {%
0 2000009.48683298
1 5.19035671704369
2 0.783654756981679
3 0.314909565247869
4 0.18282797723237
5 0.166255873151006
6 0.134098789113443
7 0.0691763214715977
8 0.0626830477478831
9 0.0911014452472739
10 0.0529665326500196
11 0.0934309159455208
12 0.0262542810642024
13 0.016855603869119
14 0.0286672767030298
15 0.0218430313879711
16 0.0207443943310774
17 0.0416990510727177
18 0.0299338365386715
19 0.0193461698941842
20 0.0348398524401277
21 0.0367187365283696
22 0.0362903977429944
23 0.0405816504603199
24 0.0252288674681357
25 0.0077644662710083
26 0.0271181646566857
27 0.0238168072865368
28 0.0151681154821325
29 0.0151844664544115
30 0.0265625229028419
31 0.0494506937296438
32 0.0220114743877243
33 0.0174793097094548
34 0.0256039494959446
35 0.0145227310069609
36 0.0309822180562881
37 0.00592531607953999
38 0.00660050635043277
39 0.00718391353357283
40 0.010885996900573
41 0.0262561620464707
42 0.0191895286058851
43 0.0221350502889347
44 0.0287991816491489
45 0.0326178438281707
46 0.0340557735520964
47 0.0377695186579871
48 0.046732880819269
49 0.0318958090096951
50 0.0189257431916797
51 0.035841628259276
52 0.0414098610070176
53 0.0176426090215031
54 0.0317536492352048
55 0.0384947952932368
56 0.0258051632331616
57 0.0248728892339056
58 0.0283229373234188
59 0.0122379864251728
60 0.0165019301425437
61 0.0257832212750526
62 0.0259895664541946
63 0.0509094941899583
64 0.0458795226069587
65 0.0349624379234345
66 0.0375280323687214
67 0.0220607732483767
68 0.0230071175709171
69 0.0279965701930056
70 0.0295523667991861
71 0.0391721121399066
72 0.0128132656312476
73 0.0119934204071416
74 0.00835740055950225
75 0.0136723911280245
76 0.0234554436198633
77 0.0119133381670167
78 0.0257466124263113
79 0.0961899024505797
80 0.0290499322740325
81 0.0357689292300256
82 0.0486426010377879
83 0.0224179548180106
84 0.0263934079073483
85 0.0212323210906647
86 0.0270467124619962
87 0.0187524938989709
88 0.0324285496842178
89 0.0194794723011561
90 0.0112027499414148
91 0.0196262867252057
92 0.0204026947008971
93 0.0284780759665116
94 0.00639889448561375
95 0.00397291337893349
96 0.0144242569752536
97 0.0220588919601779
98 0.0204232058977128
99 0.01252723600877
};
\addlegendentry{\(\dualstepsizeminimizer=\dualstepsizemaximizer=0.1\)}
\addplot [line width=2pt, orange]
table {%
0 2000009.48683298
1 0.881538683003554
2 0.249642199125332
3 0.251043208366968
4 0.231761725568245
5 0.193947028472149
6 0.206236790085025
7 0.177810871672658
8 0.219352956837116
9 0.197603326632641
10 0.243546494881033
11 0.202295706456535
12 0.171283136928307
13 0.192092307775105
14 0.202525003757439
15 0.158661656243172
16 0.17462164886646
17 0.20497154276971
18 0.188398866315267
19 0.183851128085464
20 0.199181696269222
21 0.194856216595952
22 0.174500980868696
23 0.165599700821033
24 0.12982085995805
25 0.129796934738306
26 0.125051377870762
27 0.144156690265606
28 0.139918445753525
29 0.134358760358915
30 0.121580900812628
31 0.13267861540115
32 0.143960965513147
33 0.137312473372954
34 0.149572880899662
35 0.143478660688656
36 0.0998225226130166
37 0.116667334103533
38 0.143061706417342
39 0.0813050854771119
40 0.0895270052407848
41 0.133294689903416
42 0.0878997227245144
43 0.127322633163541
44 0.110761028783031
45 0.118204672521615
46 0.0930648101616524
47 0.110726291058011
48 0.100598531730998
49 0.084002784250941
50 0.125062170313088
51 0.103432232503046
52 0.0976502052837089
53 0.101518519927797
54 0.104415552886192
55 0.0811691965624181
56 0.0837818687466409
57 0.109874521997983
58 0.132499469699652
59 0.11333902340421
60 0.0874248116223946
61 0.0988178489723073
62 0.131119218589868
63 0.0846502486557496
64 0.0974906933028205
65 0.10000561780478
66 0.107122599468246
67 0.0946738249303216
68 0.107979886029264
69 0.0661486055222486
70 0.0933206986785302
71 0.0794739559973004
72 0.0828057850529337
73 0.113717457473714
74 0.0925755183678715
75 0.0642908376102933
76 0.0744202633026643
77 0.0801832185377294
78 0.130664540108789
79 0.0519544455204037
80 0.0811846455418188
81 0.0704401709531003
82 0.0685729297686058
83 0.0898778551430968
84 0.101402281797941
85 0.0504235964709869
86 0.0897987291095918
87 0.0875574365356084
88 0.0751684694157063
89 0.0365791174812808
90 0.0392683775614939
91 0.0514015762508535
92 0.055384576069056
93 0.112863628475298
94 0.055622420753308
95 0.0948626753869815
96 0.0705050403408063
97 0.0608351264744201
98 0.110375221558729
99 0.056423407312717
};
\addlegendentry{\(\dualstepsizeminimizer=\dualstepsizemaximizer=1\)}
\end{axis}

\end{tikzpicture}

